Language2Pose: Natural Language Grounded Pose Forecasting

Generating animations from natural language sentences finds its applications in a a number of domains such as movie script visualization, virtual human animation and, robot motion planning. These sentences can describe different kinds of actions, speeds and direction of these actions, and possibly a target destination. The core modeling challenge in this language-to-pose application is how to map linguistic concepts to motion animations. In this paper, we address this multimodal problem by introducing a neural architecture called Joint Language to Pose (or JL2P), which learns a joint embedding of language and pose. This joint embedding space is learned end-to-end using a curriculum learning approach which emphasizes shorter and easier sequences first before moving to longer and harder ones. We evaluate our proposed model on a publicly available corpus of 3D pose data and human-annotated sentences. Both objective metrics and human judgment evaluation confirm that our proposed approach is able to generate more accurate animations and are deemed visually more representative by humans than other data driven approaches.

==> p3_userStudy_ablation.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{plots/userStudy_ablation.png}
  \caption{Preference scores of ablation models vs ground truth. Blue bars denote the preference percentage of models marked on the horizontal axis. \modelshorts loses human preference if the language encoder $p_e$ is switched to BERT, from LSTMs but it is still better than \baseline.}\label{fig:userstudy_ablation}
\end{figure}

==> p4_ape_time.tex <==
\begin{figure}[]
  \centering
  \includegraphics[width=0.5\textwidth]{plots/mean_ape_across_time.png}
  \caption{Plot of mean APE values across time steps for all baseline models. Each time-step is approximately 80ms long. Lower is better.}\label{fig:ape_time}
\end{figure}

==> p9_overview.tex <==
\begin{figure*}[!th]
  \centering
  \includegraphics[width=0.5\textwidth]{plots/overview.png}
  \caption{}
\end{figure*}

==> z99_table_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}c|cc|ccc@{}}
\toprule
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Language \\ Encoder \\ ($p_e$)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Feedback}}          & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average Positional Error \\ (APE) in mm\end{tabular}}}                                  \\ \cmidrule(l){2-6} 
                                                                                                 & \textbf{$\mathcal{Z}$} & \textbf{$\mathcal{C}$} & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ w/o Root\end{tabular}} & \textbf{Root}  & \textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ \end{tabular}} \\ \midrule
\textbf{LSTM}                                                                                    & $\xmark$               & $\xmark$               & 41.6                                                               & 131.1          & 49.5                                                          \\
\textbf{BERT}                                                                                    & $\xmark$               & $\xmark$               & 40.4                                                               & 129.0          & 48.2                                                          \\
\textbf{LSTM}                                                                                    & $\cmark$               & $\xmark$               & \textbf{39.9}                                                      & \textbf{126.2} & \textbf{47.5}                                                 \\
\textbf{BERT}                                                                                    & $\cmark$               & $\xmark$               & 40.9                                                               & 137.7          & 49.1                                                          \\
\textbf{LSTM}                                                                                    & $\xmark$               & $\cmark$               & 41.0                                                               & 134.3          & 49.1                                                          \\
\textbf{BERT}                                                                                    & $\xmark$               & $\cmark$               & \textbf{39.9}                                                      & \textbf{126.7} & \textbf{47.5}                                                 \\ \bottomrule
\end{tabular}
\caption{Average Positional Error (APE) for our model \modelshorts and its variants by tweaking language encoder (LSTM vs BERT) and pose decoder (\textbf{emphasizing language context} ($z \in \mathcal{Z}$) or \textbf{emphazising pose context} ($c\in \mathcal{C}$).)}\label{tab:ablation}
\end{table}
